What does a network layer hear? Analyzing hidden representations of end-to-end ASR through speech synthesis

End-to-end speech recognition systems have achieved competitive results compared to traditional systems. However, the complex transformations involved between layers given highly variable acoustic signals are hard to analyze. In this paper, we present our ASR probing model, which synthesizes speech from hidden representations of end-to-end ASR to examine the information maintain after each layer calculation. Listening to the synthesized speech, we observe gradual removal of speaker variability and noise as the layer goes deeper, which aligns with the previous studies on how deep network functions in speech recognition. This paper is the first study analyzing the end-to-end speech recognition model by demonstrating what each layer hears. Speaker verification and speech enhancement measurements on synthesized speech are also conducted to confirm our observation further.

==> figs/speaker_spec.tex <==

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer0.png}
        \caption{cnn1(layer 1)}
        \label{fig:layer1}
    \end{subfigure}
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer4.png}
        \caption{maxpool1(layer 5)}
        \label{fig:layer5}
    \end{subfigure}
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer9.png}
        \caption{maxpool2 (layer 10)}
        \label{fig:layer10}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer10.png}
        \caption{blstm1 (layer 11)}
        \label{fig:layer11}
    \end{subfigure}
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer12.png}
        \caption{blstm3 (layer 13)}
        \label{fig:layer13}
    \end{subfigure}
    \begin{subfigure}[b]{0.20\textwidth}
        \includegraphics[width=\textwidth]{pics/layer14.png}
        \caption{blstm5 (layer 15)}
        \label{fig:layer15}
    \end{subfigure}
    \caption{80-dimensional mel-spectrograms reconstructed from different layers of the VGG-LSTM ASR model.}
    \label{fig:speaker}
\end{figure*}

==> tables/archi.tex <==
\begin{table}[t]
  \centering
  \begin{subtable}[t]{1.0\linewidth}
  \centering
  \caption{VGG-LSTM.}
  \begin{tabular}{c c c c c}
    \toprule
    \textbf{Layer} & \textbf{Type} & \textbf{In} & \textbf{Out} & \textbf{Kernel Size} \\
    \midrule
    1 & cnn1     & 3   & 64  & 3x3 \\
    2 & relu1    & -   & -   &  -  \\
    3 & cnn2     & 64  & 64  & 3x3 \\
    4 & relu2    & -   & -   &  -  \\
    5 & maxpool1 & -   & -   & 2x2 \\
    6 & cnn3     & 64  & 128 & 3x3 \\
    7 & relu3    & -   &  -  &  -  \\
    8 & cnn4     & 128 & 128 & 3x3 \\
    9 & relu4    & -   &  -  &  -  \\
    10 & maxpool2 & -   & -   & 2x2 \\
    11 & blstm1   & 2560 & 320 &  - \\
    12 & blstm2   & 640 & 320 &  - \\
    13 & blstm3   & 640 & 320 &  - \\
    14 & blstm4   & 640 & 320 &  - \\
    15 & blstm5   & 640 & 320 &  - \\
    \bottomrule
  \end{tabular}
  \vspace{15pt}
  \centering
\caption{Pure LSTM.}
  \begin{tabular}{c c c c c}
    \toprule
    \textbf{Layer} & \textbf{Type} & \textbf{In} & \textbf{Out} & \textbf{Downsample} \\
    \midrule
    1  & blstm1  & 240 & 320 &  - \\
    2  & blstm2  & 640 & 320 &  2\\
    3  & blstm3  & 640 & 320 &  2 \\
    4  & blstm4  & 640 & 320 &  2 \\
    5  & blstm5  & 640 & 320 &  - \\
    \bottomrule
  \end{tabular}
\end{subtable}
\caption{Model architecture used in this work.}
\label{tab:archi}
\end{table}

==> tables/asr.tex <==
\begin{table}[b]
  \centering
  \begin{tabular}{c c c c}
    \toprule
%    \multicolumn{2}{c}{Preprocessing} &
%    \multicolumn{2}{c}{ASR}\\
    \multicolumn{1}{c}{\textbf{Param}} &
    \multicolumn{1}{c}{\textbf{Value}} &
    \multicolumn{1}{c}{\textbf{Param}} &
    \multicolumn{1}{c}{\textbf{Value}} \\
    \midrule
    Sampling rate & 16k Hz & Optimizer & SGD \\
    Pre-emphasis & 0.97    & Momentum  & 0.9  \\
    Frame length & 50ms    & Nesterov  & enabled \\
    Frame shift &  12.5ms  & Training steps & 200k \\
    Window type & Hann     & Modeling unit  & Subword \\
    Size of FFT & 2048     & Vocabulary size & 5000 \\
    Number of mels & 80    & Batch size & 24\\
    \bottomrule
  \end{tabular}
  \caption{ASR hyper-parameters.}
  \label{tab:asr}
\end{table}

==> tables/human.tex <==
\begin{table}[b]
  \centering
  \begin{tabular}{c c c c c c}
    \toprule
    \multicolumn{1}{c}{\textbf{cnn1}} &
    \multicolumn{1}{c}{\textbf{max1}} &
    \multicolumn{1}{c}{\textbf{max2}} &
    \multicolumn{1}{c}{\textbf{blstm1}} &
    \multicolumn{1}{c}{\textbf{blstm3}} &
    \multicolumn{1}{c}{\textbf{blstm5}} \\
    \midrule
    4.38\% & 4.68\% & 7.18\% & 16.48\% & 30.03\% & 48.07\% \\
    4.71\% & 5.09\% & 5.64\% & 10.27\% & 29.84\% & 47.12\% \\
    5.36\% & 7.59\% & 11.16\% & 8.93\%  & 24.55\% & 50.89\% \\
    \bottomrule
  \end{tabular}
  \caption{ASR hyper-parameters.}
  \label{tab:human}
\end{table}

